Rates and Properties of Strongly Gravitationally Lensed Supernovae and their Host Galaxies in Time-Domain Imaging Surveys

Supernovae that are strongly gravitationally lensed (gLSNe) by galaxies are powerful probes of astrophysics and cosmology that will be discovered systematically by next-generation wide-field, high-cadence imaging surveys such as the Zwicky Transient Facility (ZTF) and the Large Synoptic Survey Telescope (LSST). Here we use pixel-level simulations that include dust, observing strategy, and multiple supernova subtypes to forecast the rates and properties of gLSNe that ZTF and LSST will find. Applying the resolution-insensitive discovery strategy of Goldstein et al. (2018), we forecast that ZTF (LSST) can discover 0.02 (0.79) 91bg-like, 0.17 (5.92) 91T-like, 1.22 (47.84) Type Ia, 2.76 (88.51) Type IIP, 0.31 (12.78) Type IIL, and 0.36 (15.43) Type Ib/c gLSNe per year. We also forecast that the surveys can discover at least 3.75 (209.32) Type IIn gLSNe per year, for a total of at least 8.60 (380.60) gLSNe per year under fiducial observing strategies. ZTF gLSNe have a median $z_s=0.9$, $z_l=0.35$, $\mu_\mathrm{tot}=30$, $\Delta t_\mathrm{max}= 10$ days, $\min(\theta)= 0.25^{\prime\prime}$, and $N_\mathrm{img} = 4$. LSST gLSNe are less compact and less magnified, with a median $z_s=1.0$, $z_l=0.4$, $\mu_\mathrm{tot}\approx6$, $\Delta t_\mathrm{max} = 25$ days, $\min(\theta)=0.6^{\prime\prime}$, and $N_\mathrm{img} = 2$. As the properties of lensed host galaxy arcs provide critical information for lens mass modeling, we develop a model of the supernova--host galaxy connection and use it to simulate realistic images of the supernova--host--lens systems. We find that the vast majority of gLSN host galaxies will be multiply imaged, enabling detailed constraints on lens models with sufficiently deep high-resolution imaging taken after the supernova has faded. We release the results of our simulations to the public as catalogs at this URL: http://portal.nersc.gov/project/astro250/glsne/.

==> shortcuts.tex <==
\newcommand{\rem}[1]{\textcolor{red}{\textbf{--- #1 ---}}}
\newcommand{\needref}{\rem{REF}}
\newcommand{\snia}{{\rm SN~Ia}}
\newcommand{\sneia}{{\rm SNe~Ia}}
\newcommand{\q}[1]{{\tt #1}}
\newcommand{\nsn}{\rem{XX}}
\newcommand{\Nifs}{\ensuremath{^{56}\mathrm{Ni}}}
\newcommand{\Nife}{\ensuremath{^{58}\mathrm{Ni}}}
\newcommand{\Cofs}{\ensuremath{^{56}\mathrm{Co}}}
\newcommand{\Fefs}{\ensuremath{^{56}\mathrm{Fe}}}
\newcommand{\Feff}{\ensuremath{^{54}\mathrm{Fe}}}
\newcommand{\Fefe}{\ensuremath{^{58}\mathrm{Fe}}}
\newcommand{\mej}{\ensuremath{M_{\rm Ej}}}
\newcommand{\mni}{\ensuremath{M_{^{56}\mathrm{Ni}}}}
\newcommand{\mfe}{\ensuremath{M_{^{54}\mathrm{Fe}}}}
\newcommand{\mco}{\ensuremath{M_{\rm CO}}}
\newcommand{\mime}{\ensuremath{M_{\rm IME}}}
\newcommand{\msun}{{\ensuremath{M_{\odot}}}}
\newcommand{\Msun}{{\ensuremath{M_{\odot}}}}
\newcommand{\zsun}{\ensuremath{Z_\odot}}
\newcommand{\texp}{\ensuremath{t_{\mathrm{exp}}}}
\newcommand{\Mni}{\ensuremath{M_{\mathrm{Ni}}}}
\newcommand{\Mfe}{\ensuremath{M_{\mathrm{Fe}}}}
\newcommand{\Mime}{\ensuremath{M_{\mathrm{IME}}}}
\newcommand{\Mburn}{{\ensuremath{\mathrm{M}_{\mathrm{burn}}}}}
\newcommand{\Mej}{\ensuremath{M_{\mathrm{Ej}}}}
\newcommand{\cgsdensity}{\ensuremath{\mathrm{g~cm}^{-3}}}
\newcommand{\NiCent}{\ensuremath{M^c_{\mathrm{Ni}}}}
\newcommand{\Mch}{{\ensuremath{M_\mathrm{ch}}}}
\newcommand{\KE}{\ensuremath{E_K}}
\newcommand{\Mb}{\ensuremath{M_B}}
\newcommand{\lamopt}{\ensuremath{\lambda_{\mathrm{opt}}}}
\newcommand{\dmf}{\ensuremath{\Delta M_{15}}}
\newcommand{\dmfb}{\ensuremath{\Delta M_{15}(B)}}
\newcommand{\dmfmin}{\ensuremath{\Delta  M_{15,\mathrm{min}}}}
\newcommand{\dmfmax}{\ensuremath{\Delta  M_{15,\mathrm{max}}}}
\newcommand{\phiNi}{{\ensuremath{\phi_\mathrm{Ni}}}}
\newcommand{\epth}{{\ensuremath{\epsilon_{\rm th}}}}
\newcommand{\MCcode}{\texttt{SEDONA}}
\newcommand{\MLcode}{\texttt{MULES}}
\newcommand{\kms}{\ensuremath{\mathrm{km~s}^{-1}}}
\newcommand{\zcmb}{\ensuremath{z_{\mathrm{CMB}}}}
\newcommand{\zhelio}{\ensuremath{z_{\mathrm{Helio}}}}
\newcommand{\Model}{BOLT}
\newcommand{\Simple}{\q{SIMPLE}}
\newcommand{\Nmix}{\ensuremath{N_{\mathrm{mix}}}}
\newcommand{\sne}{{\rm SNe}}
\newcommand{\dmfbol}{\ensuremath{\Delta M_{15}(\rm{bol})}}
\newcommand{\about}{\ensuremath{\sim}}
\newcommand{\sglsneia}{\sneia-SL}
\newcommand{\sglsnia}{\snia-SL}
\newcommand{\dt}{\ensuremath{\Delta t}}
\newcommand{\jwst}{\textit{JWST}}
\newcommand{\sneiip}{SNe~IIP}
\newcommand{\Crfe}{\ensuremath{^{48}\mathrm{Cr}}}
\newcommand{\Vfe}{\ensuremath{^{48}\mathrm{V}}}
\newcommand{\Tife}{\ensuremath{^{48}\mathrm{Ti}}}
\newcommand{\lcdm}{\ensuremath{\Lambda}CDM}
\newcommand{\silicon}{\ensuremath{^{28}\mathrm{Si}}}
\newcommand{\sulfur}{\ensuremath{^{32}\mathrm{S}}}
\newcommand{\argon}{\ensuremath{^{36}\mathrm{Ar}}}
\newcommand{\calcium}{\ensuremath{^{40}\mathrm{Ca}}}
\newcommand{\hst}{\textit{HST}}

